Attention Strategies for Multi-Source Sequence-to-Sequence Learning

Modeling attention in neural multi-source sequence-to-sequence learning remains a relatively unexplored area, despite its usefulness in tasks that incorporate multiple source languages or modalities. We propose two novel approaches to combine the outputs of attention mechanisms over each source sequence, flat and hierarchical. We compare the proposed methods with existing techniques and present results of systematic evaluation of those methods on the WMT16 Multimodal Translation and Automatic Post-editing tasks. We show that the proposed methods achieve competitive results on both tasks.

==> gnuplot-lua-tikz-common.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%     Common style file for TeX, LaTeX and ConTeXt
%%  
%%  It is associated with the 'gnuplot.lua' script, and usually generated
%%  automatically. So take care whenever you make any changes!
%%

% check for the correct TikZ version
\def\gpchecktikzversion#1.#2\relax{%
\ifnum#1<2%
  \errmessage{PGF/TikZ version >= 2.0 is required!}%
\fi}
\expandafter\gpchecktikzversion\pgfversion\relax

% FIXME: is there a more elegant way to determine the output format?

\def\pgfsysdriver@a{pgfsys-dvi.def}       % ps
\def\pgfsysdriver@b{pgfsys-dvipdfm.def}   % pdf
\def\pgfsysdriver@c{pgfsys-dvipdfmx.def}  % pdf
\def\pgfsysdriver@d{pgfsys-dvips.def}     % ps
\def\pgfsysdriver@e{pgfsys-pdftex.def}    % pdf
\def\pgfsysdriver@f{pgfsys-tex4ht.def}    % html
\def\pgfsysdriver@g{pgfsys-textures.def}  % ps
\def\pgfsysdriver@h{pgfsys-vtex.def}      % ps
\def\pgfsysdriver@i{pgfsys-xetex.def}     % pdf

\newif\ifgppdfout\gppdfoutfalse
\newif\ifgppsout\gppsoutfalse

\ifx\pgfsysdriver\pgfsysdriver@a
  \gppsouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@b
  \gppdfouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@c
  \gppdfouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@d
  \gppsouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@e
  \gppdfouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@f
  % tex4ht
\else\ifx\pgfsysdriver\pgfsysdriver@g
  \gppsouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@h
  \gppsouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@i
  \gppdfouttrue
\fi\fi\fi\fi\fi\fi\fi\fi\fi

% uncomment the following lines to make font values "appendable"
% and if you are really sure about that ;-)
% \pgfkeyslet{/tikz/font/.@cmd}{\undefined}
% \tikzset{font/.initial={}}
% \def\tikz@textfont{\pgfkeysvalueof{/tikz/font}}

%
% image related stuff
%
\def\gp@rawimage@pdf#1#2#3#4#5#6{%
  \def\gp@tempa{cmyk}%
  \def\gp@tempb{#1}%
  \ifx\gp@tempa\gp@tempb%
    \def\gp@temp{/CMYK}%
  \else%
    \def\gp@temp{/RGB}%
  \fi%
  \pgf@sys@bp{#4}\pgfsysprotocol@literalbuffered{0 0}\pgf@sys@bp{#5}%
  \pgfsysprotocol@literalbuffered{0 0 cm}%
  \pgfsysprotocol@literalbuffered{BI /W #2 /H #3 /CS \gp@temp}%
  \pgfsysprotocol@literalbuffered{/BPC 8 /F /AHx ID}%
  \pgfsysprotocol@literal{#6 > EI}%
}
\def\gp@rawimage@ps#1#2#3#4#5#6{%
  \def\gp@tempa{cmyk}%
  \def\gp@tempb{#1}%
  \ifx\gp@tempa\gp@tempb%
    \def\gp@temp{4}%
  \else%
    \def\gp@temp{3}%
  \fi%
  \pgfsysprotocol@literalbuffered{0 0 translate}%
  \pgf@sys@bp{#4}\pgf@sys@bp{#5}\pgfsysprotocol@literalbuffered{scale}%
  \pgfsysprotocol@literalbuffered{#2 #3 8 [#2 0 0 -#3 0 #3]}%
  \pgfsysprotocol@literalbuffered{currentfile /ASCIIHexDecode filter}%
  \pgfsysprotocol@literalbuffered{false \gp@temp\space colorimage}%
  \pgfsysprotocol@literal{#6 >}%
}
\def\gp@rawimage@html#1#2#3#4#5#6{%
% FIXME: print a warning message here
}

\ifgppdfout
  \def\gp@rawimage{\gp@rawimage@pdf}
\else
  \ifgppsout
    \def\gp@rawimage{\gp@rawimage@ps}
  \else
    \def\gp@rawimage{\gp@rawimage@html}
  \fi
\fi


\def\gploadimage#1#2#3#4#5{%
  \pgftext[left,bottom,x=#1cm,y=#2cm] {\pgfimage[interpolate=false,width=#3cm,height=#4cm]{#5}};%
}

\def\gp@set@size#1{%
  \def\gp@image@size{#1}%
}

\def\gp@rawimage@#1#2#3#4#5#6#7#8{
  \tikz@scan@one@point\gp@set@size(#6,#7)\relax%
  \tikz@scan@one@point\pgftransformshift(#2,#3)\relax%
  \pgftext {%
    \pgfsys@beginpurepicture%
    \gp@image@size% fill \pgf@x and \pgf@y
    \gp@rawimage{#1}{#4}{#5}{\pgf@x}{\pgf@y}{#8}%
    \pgfsys@endpurepicture%
  }%
}

%% \gprawimage{color model}{xcoord}{ycoord}{# of xpixel}{# of ypixel}{xsize}{ysize}{rgb/cmyk hex data RRGGBB/CCMMYYKK ...}{file name}
%% color model is 'cmyk' or 'rgb' (default)
\def\gprawimage#1#2#3#4#5#6#7#8#9{%
  \ifx&#9&%
    \gp@rawimage@{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}
  \else
    \ifgppsout
      \gp@rawimage@{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}
    \else
      \gploadimage{#2}{#3}{#6}{#7}{#9}
    \fi
  \fi
}

%
% gnuplottex comapatibility
% (see http://www.ctan.org/tex-archive/help/Catalogue/entries/gnuplottex.html)
%

\def\gnuplottexextension@lua{\string tex}
\def\gnuplottexextension@tikz{\string tex}

%
% gnuplot variables getter and setter
%

\def\gpsetvar#1#2{%
  \expandafter\xdef\csname gp@var@#1\endcsname{#2}
}

\def\gpgetvar#1{%
  \csname gp@var@#1\endcsname %
}

%
% some wrapper code
%

% short for a filled path
\def\gpfill#1{\path[line width=0.1\gpbaselw,draw,fill,#1]}

% short for changing the line width
\def\gpsetlinewidth#1{\pgfsetlinewidth{#1\gpbaselw}}

% short for changing the line type
\def\gpsetlinetype#1{\tikzset{gp path/.style={#1,#1 add}}}

% short for changing the dash pattern
\def\gpsetdashtype#1{\tikzset{gp path/.append style={#1}}}

% short for changing the point size
\def\gpsetpointsize#1{\tikzset{gp point/.style={mark size=#1\gpbasems}}}

% wrapper for color settings
\def\gpcolor#1{\tikzset{global #1}}
\tikzset{rgb color/.code={\pgfutil@definecolor{.}{rgb}{#1}\tikzset{color=.}}}
\tikzset{global rgb color/.code={\pgfutil@definecolor{.}{rgb}{#1}\pgfutil@color{.}}}
\tikzset{global color/.code={\pgfutil@color{#1}}}

% prevent plot mark distortions due to changes in the PGF transformation matrix
% use `\gpscalepointstrue' and `\gpscalepointsfalse' for enabling and disabling
% point scaling
%
\newif\ifgpscalepoints
\tikzset{gp shift only/.style={%
  \ifgpscalepoints\else shift only\fi%
}}
\def\gppoint#1#2{%
  \path[solid] plot[only marks,gp point,mark options={gp shift only},#1] coordinates {#2};%
}


%
% char size calculation, that might be used with gnuplottex
%
% Example code (needs gnuplottex.sty):
%
%    % calculate the char size when the "gnuplot" style is used
%    \tikzset{gnuplot/.append style={execute at begin picture=\gpcalccharsize}}
%
%    \tikzset{gnuplot/.append style={font=\ttfamily\footnotesize}}
%
%    \begin{tikzpicture}[gnuplot]
%      \begin{gnuplot}[terminal=lua,%
%          terminaloptions={tikz solid nopic charsize \the\gphcharsize,\the\gpvcharsize}]
%        test
%      \end{gnuplot}
%    \end{tikzpicture}
%
%%%
% The `\gpcalccharsize' command fills the lengths \gpvcharsize and \gphcharsize with
% the values of the current default font used within nodes and is meant to be called
% within a tikzpicture environment.
% 
\newdimen\gpvcharsize
\newdimen\gphcharsize
\def\gpcalccharsize{%
  \pgfinterruptboundingbox%
  \pgfsys@begininvisible%
  \node at (0,0) {%
    \global\gphcharsize=1.05\fontcharwd\font`0%
    \global\gpvcharsize=1.05\fontcharht\font`0%
    \global\advance\gpvcharsize by 1.05\fontchardp\font`g%
  };%
  \pgfsys@endinvisible%
  \endpgfinterruptboundingbox%
}

%
%  define a rectangular node in tikz e.g. for the plot area
%
%  #1 node name
%  #2 coordinate of "south west"
%  #3 coordinate of "north east"
%
\def\gpdefrectangularnode#1#2#3{%
  \expandafter\gdef\csname pgf@sh@ns@#1\endcsname{rectangle}
  \expandafter\gdef\csname pgf@sh@np@#1\endcsname{%
    \def\southwest{#2}%
    \def\northeast{#3}%
  }
  \pgfgettransform\pgf@temp%
  % once it is defined, no more transformations will be applied, I hope
  \expandafter\xdef\csname pgf@sh@nt@#1\endcsname{\pgf@temp}%
  \expandafter\xdef\csname pgf@sh@pi@#1\endcsname{\pgfpictureid}%
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%  You may want to adapt the following to fit your needs (in your 
%%  individual style file and/or within your document).
%%

%
% style for every plot
%
\tikzset{gnuplot/.style={%
  >=stealth',%
  line cap=round,%
  line join=round,%
}}

\tikzset{gp node left/.style={anchor=mid west,yshift=-.12ex}}
\tikzset{gp node center/.style={anchor=mid,yshift=-.12ex}}
\tikzset{gp node right/.style={anchor=mid east,yshift=-.12ex}}

% basic plot mark size (points)
\newdimen\gpbasems
\gpbasems=.4pt

% basic linewidth
\newdimen\gpbaselw
\gpbaselw=.4pt

% this is the default color for pattern backgrounds
\colorlet{gpbgfillcolor}{white}

% set background color and fill color
\def\gpsetbgcolor#1{%
  \pgfutil@definecolor{gpbgfillcolor}{rgb}{#1}%
  \tikzset{tight background,background rectangle/.style={fill=gpbgfillcolor},show background rectangle}%
}

% this should reverse the normal text node presets, for the
% later referencing as described below
\tikzset{gp refnode/.style={coordinate,yshift=.12ex}}

% to add an empty label with the referenceable name "my node"
% to the plot, just add the following line to your gnuplot
% file:
%
% set label "" at 1,1 font ",gp refnode,name=my node"
%

% enlargement of the bounding box in standalone mode (only used by LaTeX/ConTeXt)
\def\gpbboxborder{0mm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%  The following TikZ-styles are derived from the 'pgf.styles.*' tables
%%  in the Lua script.
%%  To change the number of used styles you should change them there and
%%  regenerate this style file.
%%

% arrow styles settings
\tikzset{gp arrow 1/.style={>=latex}}
\tikzset{gp arrow 2/.style={>=angle 90}}
\tikzset{gp arrow 3/.style={>=angle 60}}
\tikzset{gp arrow 4/.style={>=angle 45}}
\tikzset{gp arrow 5/.style={>=o}}
\tikzset{gp arrow 6/.style={>=*}}
\tikzset{gp arrow 7/.style={>=diamond}}
\tikzset{gp arrow 8/.style={>=open diamond}}
\tikzset{gp arrow 9/.style={>={]}}}
\tikzset{gp arrow 10/.style={>={[}}}
\tikzset{gp arrow 11/.style={>=)}}
\tikzset{gp arrow 12/.style={>=(}}

% plotmark settings
\tikzset{gp mark 0/.style={mark size=.5\pgflinewidth,mark=*}}
\tikzset{gp mark 1/.style={mark=+}}
\tikzset{gp mark 2/.style={mark=x}}
\tikzset{gp mark 3/.style={mark=star}}
\tikzset{gp mark 4/.style={mark=square}}
\tikzset{gp mark 5/.style={mark=square*}}
\tikzset{gp mark 6/.style={mark=o}}
\tikzset{gp mark 7/.style={mark=*}}
\tikzset{gp mark 8/.style={mark=triangle}}
\tikzset{gp mark 9/.style={mark=triangle*}}
\tikzset{gp mark 10/.style={mark=triangle,every mark/.append style={rotate=180}}}
\tikzset{gp mark 11/.style={mark=triangle*,every mark/.append style={rotate=180}}}
\tikzset{gp mark 12/.style={mark=diamond}}
\tikzset{gp mark 13/.style={mark=diamond*}}
\tikzset{gp mark 14/.style={mark=otimes}}
\tikzset{gp mark 15/.style={mark=oplus}}

% pattern settings
\tikzset{gp pattern 0/.style={white}}
\tikzset{gp pattern 1/.style={pattern=north east lines}}
\tikzset{gp pattern 2/.style={pattern=north west lines}}
\tikzset{gp pattern 3/.style={pattern=crosshatch}}
\tikzset{gp pattern 4/.style={pattern=grid}}
\tikzset{gp pattern 5/.style={pattern=vertical lines}}
\tikzset{gp pattern 6/.style={pattern=horizontal lines}}
\tikzset{gp pattern 7/.style={pattern=dots}}
\tikzset{gp pattern 8/.style={pattern=crosshatch dots}}
\tikzset{gp pattern 9/.style={pattern=fivepointed stars}}
\tikzset{gp pattern 10/.style={pattern=sixpointed stars}}
\tikzset{gp pattern 11/.style={pattern=bricks}}

% if the 'tikzplot' option is used the corresponding lines will be smoothed by default
\tikzset{gp plot axes/.style=}
\tikzset{gp plot border/.style=}
\tikzset{gp plot 0/.style=smooth}
\tikzset{gp plot 1/.style=smooth}
\tikzset{gp plot 2/.style=smooth}
\tikzset{gp plot 3/.style=smooth}
\tikzset{gp plot 4/.style=smooth}
\tikzset{gp plot 5/.style=smooth}
\tikzset{gp plot 6/.style=smooth}
\tikzset{gp plot 7/.style=smooth}

% linestyle settings
\tikzset{gp lt axes/.style=dotted}
\tikzset{gp lt border/.style=solid}

% linestyle "addon" settings for overwriting a default linestyle within the
% TeX document via eg. \tikzset{gp lt plot 1 add/.style={fill=black,draw=none}} etc.
\tikzset{gp lt axes add/.style={}}
\tikzset{gp lt border add/.style={}}
\tikzset{gp lt plot 0 add/.style={}}
\tikzset{gp lt plot 1 add/.style={}}
\tikzset{gp lt plot 2 add/.style={}}
\tikzset{gp lt plot 3 add/.style={}}
\tikzset{gp lt plot 4 add/.style={}}
\tikzset{gp lt plot 5 add/.style={}}
\tikzset{gp lt plot 6 add/.style={}}
\tikzset{gp lt plot 7 add/.style={}}
\tikzset{gp lt plot 0/.style={}}
\tikzset{gp lt plot 1/.style={}}
\tikzset{gp lt plot 2/.style={}}
\tikzset{gp lt plot 3/.style={}}
\tikzset{gp lt plot 4/.style={}}
\tikzset{gp lt plot 5/.style={}}
\tikzset{gp lt plot 6/.style={}}
\tikzset{gp lt plot 7/.style={}}

% linestyle color settings
\colorlet{gp lt color axes}{black!30}
\colorlet{gp lt color border}{black}

% dash type settings
% Define this as a macro so that the dash patterns expand later with the current \pgflinewidth.
\def\gpdashlength{\pgflinewidth}
\tikzset{gp dt 0/.style={solid}}
\tikzset{gp dt 1/.style={solid}}
\tikzset{gp dt 2/.style={dash pattern=on 7.5*\gpdashlength off 7.5*\gpdashlength}}
\tikzset{gp dt 3/.style={dash pattern=on 3.75*\gpdashlength off 5.625*\gpdashlength}}
\tikzset{gp dt 4/.style={dash pattern=on 1*\gpdashlength off 2.8125*\gpdashlength}}
\tikzset{gp dt 5/.style={dash pattern=on 11.25*\gpdashlength off 3.75*\gpdashlength on 1*\gpdashlength off 3.75*\gpdashlength}}
\tikzset{gp dt 6/.style={dash pattern=on 5.625*\gpdashlength off 5.625*\gpdashlength on 1*\gpdashlength off 5.625*\gpdashlength}}
\tikzset{gp dt 7/.style={dash pattern=on 3.75*\gpdashlength off 3.75*\gpdashlength on 3.75*\gpdashlength off 11.25*\gpdashlength}}
\tikzset{gp dt 8/.style={dash pattern=on 1*\gpdashlength off 3.75*\gpdashlength on 11.25*\gpdashlength off 3.75*\gpdashlength on 1*\gpdashlength off 3.75*\gpdashlength}}
\tikzset{gp dt solid/.style={solid}}
\tikzset{gp dt axes/.style={dotted}}

% command for switching to colored lines
\def\gpcoloredlines{%
  \colorlet{gp lt color 0}{red}%
  \colorlet{gp lt color 1}{green}%
  \colorlet{gp lt color 2}{blue}%
  \colorlet{gp lt color 3}{magenta}%
  \colorlet{gp lt color 4}{cyan}%
  \colorlet{gp lt color 5}{yellow}%
  \colorlet{gp lt color 6}{orange}%
  \colorlet{gp lt color 7}{purple}%
}

% command for switching to monochrome (black) lines
\def\gpmonochromelines{%
  \colorlet{gp lt color 0}{black}%
  \colorlet{gp lt color 1}{black}%
  \colorlet{gp lt color 2}{black}%
  \colorlet{gp lt color 3}{black}%
  \colorlet{gp lt color 4}{black}%
  \colorlet{gp lt color 5}{black}%
  \colorlet{gp lt color 6}{black}%
  \colorlet{gp lt color 7}{black}%
}

%
% some initialisations
%
% by default all lines will be colored
\gpcoloredlines
\gpsetpointsize{4}
\gpsetlinetype{gp lt solid}
\gpscalepointsfalse
\endinput

